Few-Shot Adaptation of Pre-Trained Networks for Domain Shift

Deep networks are prone to performance degradation when there is a domain shift between the source (training) data and target (test) data. Recent test-time adaptation methods update batch normalization layers of pre-trained source models deployed in new target environments with streaming data to mitigate such performance degradation. Although such methods can adapt on-the-fly without first collecting a large target domain dataset, their performance is dependent on streaming conditions such as mini-batch size and class-distribution, which can be unpredictable in practice. In this work, we propose a framework for few-shot domain adaptation to address the practical challenges of data-efficient adaptation. Specifically, we propose a constrained optimization of feature normalization statistics in pre-trained source models supervised by a small support set from the target domain. Our method is easy to implement and improves source model performance with as few as one sample per class for classification tasks. Extensive experiments on 5 cross-domain classification and 4 semantic segmentation datasets show that our method achieves more accurate and reliable performance than test-time adaptation, while not being constrained by streaming conditions.

==> tables/full_results_comparison_source_free_few_shot_all_classifiers.tex <==
\begin{table*}[ht]
\centering
\begin{adjustbox}{max width=0.8\textwidth}
\setlength\tabcolsep{4pt} % default value: 6pt
\begin{tabular}{*{10}{l}}
\toprule[1pt]\midrule[0.3pt]
\textbf{Method}             & \multicolumn{3}{c}{\textbf{PACS-Art}}  & \multicolumn{3}{c}{\textbf{PACS-Cartoon}}  & \multicolumn{3}{c}{\textbf{PACS-Photo}} \\ \cmidrule{2-10}
\multicolumn{1}{r}{$k=$}    & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{5} & \multicolumn{1}{c}{10}
                            & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{5} & \multicolumn{1}{c}{10}
                            & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{5} & \multicolumn{1}{c}{10} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} 
AdaBN                       & 80.7 \rpm 2.0 & 84.5 \rpm 0.7 & 85.0 \rpm 0.6            & 79.9 \rpm 0.9 & 83.2 \rpm 0.8 & 83.5 \rpm 0.8                
                            & 95.2 \rpm 0.6 & 96.0 \rpm 0.8 & 96.0 \rpm 0.7\\
finetune BN                 & 74.2 \rpm 3.6 & 80.9 \rpm 0.9 & 83.2 \rpm 1.4            & 77.9 \rpm 1.8 & 82.0 \rpm 1.8 & 83.1 \rpm 1.4                
                            & 92.4 \rpm 0.6 & 95.9 \rpm 0.7 & 96.2 \rpm 0.5 \\
finetune classifier         & 81.7 \rpm 0.7 & 83.7 \rpm 0.6 & 84.2 \rpm 0.3            & 79.2 \rpm 0.6 & 80.5 \rpm 0.6 & 80.5 \rpm 0.6                
                            & 95.6 \rpm 0.6 & 96.0 \rpm 0.3 & 96.1 \rpm 0.3 \\
finetune feat. extractor    & \textbf{83.3 \rpm 0.8} & 86.1 \rpm 1.3 & 86.1 \rpm 1.0            & \textbf{81.8 \rpm 1.0} & 84.0 \rpm 1.5 & 85.4 \rpm 0.8                
                            & \underline{95.9 \rpm 0.6} & 96.4 \rpm 0.5 & 96.6 \rpm 0.7 \\
$L^2$                       & \textbf{83.3 \rpm 0.9} & \textbf{85.8 \rpm 0.9} & 85.6 \rpm 0.8            & \textbf{81.8 \rpm 0.7} & 83.4 \rpm 0.4 & 84.1 \rpm 0.9                
                            & \textbf{96.1 \rpm 0.4} & 96.6 \rpm 0.5 & 96.4 \rpm 0.6 \\
$L^2$-SP                    & \textbf{83.3 \rpm 0.9} & \textbf{85.8 \rpm 0.9} & 85.6 \rpm 0.8            & \textbf{81.8 \rpm 0.7} & 83.4 \rpm 0.4 & 84.1 \rpm 0.9               
                            & \textbf{96.1 \rpm 0.4} & 96.6 \rpm 0.5 & 96.4 \rpm 0.6 \\ 
DELTA                       & \textbf{83.3 \rpm 1.0} & \textbf{85.8 \rpm 0.8} & 85.6 \rpm 0.7            & \textbf{81.8 \rpm 0.7} & 83.3 \rpm 0.3 & 83.8 \rpm 0.9               
                            & \textbf{96.1 \rpm 0.4} & \underline{96.7 \rpm 0.5} & 96.5 \rpm 0.7 \\
Late Fusion                 & \underline{83.0 \rpm 0.6} & 83.8 \rpm 0.7 & 83.8 \rpm 0.5            & 79.8 \rpm 0.2 & 79.9 \rpm 0.5 & 79.7 \rpm 0.6                
                            & 95.8 \rpm 0.4 & 95.9 \rpm 0.3 & 96.0 \rpm 0.2 \\
FLUTE                       & 67.0 \rpm 9.7 & 83.6 \rpm 3.0 & \underline{87.2 \rpm 0.8}            & 73.5 \rpm 6.4 & \underline{84.7 \rpm 0.7} & \underline{86.1 \rpm 0.5}                
                            & 90.3 \rpm 4.1 & 96.3 \rpm 0.9 & \underline{97.2 \rpm 0.2} \\ \midrule
LCCS (SC)          & 82.2 \rpm 0.9 & 84.9 \rpm 0.6 & 85.0 \rpm 1.7            & \underline{80.4 \rpm 0.9} & 82.8 \rpm 0.8 & 83.1 \rpm 0.8               
                            & \underline{95.9 \rpm 0.6} & 96.4 \rpm 0.3 & 96.6 \rpm 0.4 \\
LCCS (FC)          & 80.7 \rpm 0.9 & 84.4 \rpm 1.0 & 85.0 \rpm 1.0            & 79.7 \rpm 1.2 & 83.0 \rpm 0.8 & 83.3 \rpm 0.9                
                            & \underline{95.9 \rpm 0.5} & 96.3 \rpm 0.4 & 96.5 \rpm 0.6 \\
LCCS (NCC)         & 69.8 \rpm 6.2 & \underline{85.7 \rpm 1.2} & \textbf{87.7 \rpm 1.0}            & 73.9 \rpm 6.6 & \textbf{85.5 \rpm 0.9} & \textbf{86.9 \rpm 0.6}               
                            & 92.0 \rpm 2.2 & \textbf{97.2 \rpm 0.2} & \textbf{97.5 \rpm 0.3} \\
\midrule[0.3pt]\bottomrule[1pt]
\end{tabular}
\end{adjustbox}

\medskip

\begin{adjustbox}{max width=0.8\textwidth}
\setlength\tabcolsep{4pt} % default value: 6pt
\begin{tabular}{*{10}{l}}
\toprule[1pt]\midrule[0.3pt]
\textbf{Method}             & \multicolumn{3}{c}{\textbf{PACS-Sketch}} & \multicolumn{3}{c}{\textbf{Camelyon17}}  & \multicolumn{3}{c}{\textbf{VisDA}} \\ \cmidrule{2-10}
\multicolumn{1}{r}{$k=$}    & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{5} & \multicolumn{1}{c}{10}
                            & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{5} & \multicolumn{1}{c}{10}
                            & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{5} & \multicolumn{1}{c}{10} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
AdaBN                       & 75.8 \rpm 2.8 & 78.5 \rpm 0.6 & 78.7 \rpm 0.6            & 72.9 \rpm 14.3 & 87.8 \rpm 5.4 & \underline{90.2 \rpm 1.4} 
                            & 56.5 \rpm 0.7 & 60.9 \rpm 0.7 & 61.8 \rpm 0.3 \\
finetune BN                 & 71.7 \rpm 3.1 & 78.6 \rpm 2.5 & 79.0 \rpm 2.2            & 72.6 \rpm 7.2 & 87.7 \rpm 6.2 & 90.1 \rpm 3.5              
                            & 59.1 \rpm 0.6 & 70.9 \rpm 3.0 & 74.9 \rpm 1.5 \\
finetune classifier         & 73.2 \rpm 1.1 & 74.6 \rpm 1.0 & 74.6 \rpm 1.4            & 70.5 \rpm 6.1 & 70.4 \rpm 6.1 & 70.5 \rpm 6.0              
                            & \underline{67.6 \rpm 1.4} & 69.7 \rpm 0.9 & 77.4 \rpm 0.6 \\
finetune feat. extractor    & 73.4 \rpm 5.5 & 77.5 \rpm 2.5 & 76.3 \rpm 1.6            & \underline{79.3 \rpm 11.0} & 86.5 \rpm 5.4 & 88.3 \rpm 4.4 
                            & 67.3 \rpm 0.7 & 68.4 \rpm 0.4 & 74.7 \rpm 0.7 \\
$L^2$                       & 76.5 \rpm 2.2 & 77.5 \rpm 2.2 & 76.3 \rpm 1.1            & \textbf{79.6 \rpm 8.3} & 88.2 \rpm 3.8 & 89.5 \rpm 2.8 
                            & 66.0 \rpm 0.6 & 66.4 \rpm 0.5 & 69.6 \rpm 0.5 \\
$L^2$-SP                    & 76.5 \rpm 2.2 & 77.5 \rpm 2.2 & 76.3 \rpm 1.1            & \textbf{79.6 \rpm 8.3} & 88.2 \rpm 3.8 & 89.5 \rpm 2.8 
                            & 66.0 \rpm 0.6 & 66.4 \rpm 0.5 & 69.6 \rpm 0.5 \\ 
DELTA                       & 76.6 \rpm 2.3 & 77.4 \rpm 2.1 & 75.4 \rpm 1.3            & \textbf{79.6 \rpm 8.3} & 88.2 \rpm 3.8 & 89.5 \rpm 2.8 
                            & 65.9 \rpm 0.7 & 66.5 \rpm 0.5 & 70.1 \rpm 0.6 \\
Late Fusion                 & 74.3 \rpm 1.7 & 75.1 \rpm 1.3 & 74.9 \rpm 1.1            & 70.4 \rpm 6.1 & 70.4 \rpm 6.1 & 70.5 \rpm 6.0                
                            & 67.2 \rpm 1.2 & 69.8 \rpm 1.1 & 74.5 \rpm 0.6 \\
FLUTE                       & 62.8 \rpm 9.3 & 78.7 \rpm 3.4 & 81.7 \rpm 1.5            & 73.1 \rpm 7.5 & 86.5 \rpm 7.0 & \textbf{90.9 \rpm 3.3}               
                            & 48.3 \rpm 1.9 & 67.1 \rpm 1.9 & 65.7 \rpm 1.9 \\ \midrule
LCCS (SC)          & \textbf{78.9 \rpm 3.1} & \underline{80.6 \rpm 1.6} & \underline{82.0 \rpm 1.0}            & 76.6 \rpm 12.4 & \textbf{88.6 \rpm 3.7} & 88.9 \rpm 2.9               
                            & \textbf{67.8 \rpm 1.1} & 69.5 \rpm 0.0 & 72.5 \rpm 0.2 \\
LCCS (FC)          & \underline{78.5 \rpm 2.7} & \textbf{80.7 \rpm 1.8} & 81.5 \rpm 1.0            & 77.1 \rpm 12.0 & \underline{88.4 \rpm 3.7} & 88.6 \rpm 3.0                
                            & 64.3 \rpm 2.5 & \underline{71.1 \rpm 2.3} & \underline{77.7 \rpm 0.6} \\
LCCS (NCC)         & 65.2 \rpm 11.0 & 80.0 \rpm 2.2 & \textbf{83.0 \rpm 1.1}           & 72.4 \rpm 15.9 & 88.3 \rpm 4.0 & \underline{90.2 \rpm 1.6}                
                            & 52.9 \rpm 5.4 & \textbf{76.0 \rpm 0.5} & \textbf{79.2 \rpm 0.4} \\
\midrule[0.3pt]\bottomrule[1pt]
\end{tabular}
\end{adjustbox}

\caption{Target domain classification accuracy with different classifiers: fully-connected source classifier (SC), fully-connected finetuned classifier on support set (FC), nearest-centroid classifier on support set (NCC). \label{tab:full_results_source_free_few_shot}}
%\vspace{-3mm}
\end{table*}



==> tables/pacs_select_failure_cases.tex <==
\begin{wraptable}{r}{7cm}
\centering
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{l*{4}{c}}
\toprule[1pt]\midrule[0.3pt]
\textbf{Method} & \multicolumn{2}{c}{\textbf{Small test batches}} & \multicolumn{2}{c}{\textbf{Class imbalance}} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5}
                        & size $=8$ & size $=32$    & $\rho=10$ & $\rho=100$ \\ \midrule 
Source model (MixStyle) & 83.1      & 83.1          & 79.9      & 76.9 \\
+ Test-time BN          & 78.6      & 83.3          & 78.6      & 66.6 \\
+ Tent (Adam)           & 81.1      & \underline{86.1}          & 80.0      & 67.7 \\ \midrule
+ finetune LCCS ($k=1$) & 84.5      & 84.5          & 81.3      & 78.4 \\
+ finetune LCCS ($k=5$) & \underline{87.1}      & \underline{87.1}          & \underline{84.9}      & \underline{81.9} \\
+ finetune LCCS ($k=10$)& \textbf{88.8}      & \textbf{88.8}          & \textbf{86.8}      & \textbf{84.3} \\
\midrule[0.3pt]\bottomrule[1pt]
\end{tabular}
\end{adjustbox}
\caption{PACS: Average target domain classification accuracy for evaluation settings where test-time adaptation can degrade performance. \label{tab:pacs_select_failure_cases}}

\end{wraptable}


==> tables/results_svd.tex <==
\begin{table}[htb]
\centering
\begin{adjustbox}{max width=0.7\textwidth}
\setlength\tabcolsep{4pt} % default value: 6pt
\begin{tabular}{c*{9}{l}}
\toprule[1pt]\midrule[0.3pt]
$\boldsymbol{n}$   & \multicolumn{3}{c}{\textbf{PACS}}  & \multicolumn{3}{c}{\textbf{Camelyon17}}  & \multicolumn{3}{c}{\textbf{VisDA}} \\ \cmidrule{2-10}
\multicolumn{1}{r}{$k=$}    & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{5} & \multicolumn{1}{c}{10}
                            & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{5} & \multicolumn{1}{c}{10}
                            & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{5} & \multicolumn{1}{c}{10} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
1                           & 84.5 & 85.9 & 86.3
                            & 76.1 & 87.6 & 88.7 
                            & 67.0 & 68.1 & 69.3 \\
10                          & 83.6 & 85.6 & 86.5
                            & 76.9 & 88.4 & 88.6 
                            & 67.6 & 68.9 & 71.3 \\
$k\times$ \# classes        & 83.6 & 85.7 & 86.5
                            & 76.9 & 88.4 & 88.6
                            & 67.6 & 69.2 & 72.1 \\
90\% explained variance     & 83.6 & 85.6 & 86.4
                            & 76.9 & 88.0 & 88.4
                            & 67.5 & 68.9 & 71.4\\                            
\midrule[0.3pt]\bottomrule[1pt]
\end{tabular}
\end{adjustbox}
\caption{Target domain performance with different number $n$ of support set spanning vectors. \label{tab:results_svd}}
%\vspace{-3mm}
\end{table}


